LU-Net: a multi-task network to improve the robustness of segmentation of left ventriclular structures by deep learning in 2D echocardiography

Segmentation of cardiac structures is one of the fundamental steps to estimate volumetric indices of the heart. This step is still performed semi-automatically in clinical routine, and is thus prone to inter- and intra-observer variability. Recent studies have shown that deep learning has the potential to perform fully automatic segmentation. However, the current best solutions still suffer from a lack of robustness. In this work, we introduce an end-to-end multi-task network designed to improve the overall accuracy of cardiac segmentation while enhancing the estimation of clinical indices and reducing the number of outliers. Results obtained on a large open access dataset show that our method outperforms the current best performing deep learning solution and achieved an overall segmentation accuracy lower than the intra-observer variability for the epicardial border (i.e. on average a mean absolute error of 1.5mm and a Hausdorff distance of 5.1mm) with 11% of outliers. Moreover, we demonstrate that our method can closely reproduce the expert analysis for the end-diastolic and end-systolic left ventricular volumes, with a mean correlation of 0.96 and a mean absolute error of 7.6ml. Concerning the ejection fraction of the left ventricle, results are more contrasted with a mean correlation coefficient of 0.83 and an absolute mean error of 5.0%, producing scores that are slightly below the intra-observer margin. Based on this observation, areas for improvement are suggested.

==> sections/introduction_new.tex <==
\section{Introduction}
\label{sec:introduction}

Analysis of 2D echocardiographic images based on the measurement of cardiac morphology and function is essential for diagnosis. Low-level image processing such as segmentation and tracking enable to extract and interpret clinical indices, among which the volume of the left ventricle and the corresponding ejection fraction (\LVef) are among the most commonly used. The extraction of such measures requires accurate delineation of the left ventricular endocardium (\LVendo) at both end diastole (ED) and end systole (ES). However, these indices are subject to controversy due to a lack of reproducibility. Indeed, there is a significant variability in the measurement of the values extracted from the ultrasound images from an inter-expert, intra-expert and inter-equipment perspective. The inherent difficulties for segmenting echocardiographic images are well documented: \emph{i)} poor contrast between the myocardium and the blood pool; \emph{ii)} brightness inhomogeneities; \emph{iii)} variation in the speckle pattern along the myocardium, due to the orientation of the cardiac probe with respect to the tissue; \emph{iv)} presence of trabeculae and papillary muscles with intensities similar to the myocardium; \emph{v)} significant tissue echogenicity variability within the population; \emph{vi)} shape, intensity and motion variability across patients and pathologies.

\subsection{\modified{Related works}}
\label{sec:related_works}

\modified{
Numerous studies have been conducted for more than 30 years to make automatic measurements of the \LVendo~and \LVef~indices robust and reliable in echocardiographic imaging. Traditional methods can be classified into 2 categories: weak prior versus strong prior. The first group includes weak assumptions such as spatial, intensity or motion information and corresponds to image-based techniques \cite{Wang2014}, motion-based methods \cite{Smistad2014}, deformable models \cite{Barbosa2014,Wang2014} or graph-based approaches \cite{Bernier2014}. The second group uses approaches with strong priors including active appearance models \cite{Vanstralen2014}, atlas-based methods \cite{Oktay2014} and machine learning algorithms \cite{Milletari2014,Keraudren2014,Domingos2014}. Most of these approaches relies on handcrafted features which can be considered as an over-simplistic source of information.}

\modified{
Supervised deep learning methods rely on much more flexible models that go beyond this limitation. By definition these techniques are optimal to the data they are trained on. Such approaches have been applied in the context of left ventricular structures segmentation. In 2012, Carneiro \etal exploited deep belief networks and the decoupling of rigid and nonrigid classifiers to improve robustness in terms of image conditions and shape variability~\cite{Carneiro2012}. Later, Chen \etal used transfer learning from cross domain to enhance feature representation~\cite{Chen2016}. In parallel, Smistad \etal showed that the \unet~method~\cite{Ronneberger2015} could be trained with the output of a \sota~deformable model to successfully segment the left ventricle in 2D ultrasound images \cite{Smistad2017}. Oktay \etal further extended a \unet~base model so that its segmentation output is constrained to fit a non-linear compact representation of the underlying anatomy derived from an auto-encoder network~\cite{Oktay2018}. Recently, Bernard \etal showed that a simple \unet~model learned from a large annotated database produces accurate results that are much better than the \sota, on average lower than the inter-observer variability and close but still above the intra-observer variability with 18\% of outliers.}

\modified{Deep learning methods based on regression models without intermediate segmentation have also been studied to directly estimate clinical indices from cine-MR and echocardiographic sequences \cite{Peng2016,Xue2017,Ge2019}. In this context, the work produced by Ge \etal is among the most advanced studies \cite{Ge2019}. Based on a Res-circle network, their \mbox{PV-LVNet} model embeds both subject features and temporal changes to effectively perform localization, cropping and clinical indices regression. Although this type of method appears to give promising results, the fact that it does not produce segmentation outputs can be considered as a weakness. Indeed, segmentation contours are largely used by cardiologists to visually control the quality of the computed clinical indices. We therefore decided to focus in this article on the improvement of left ventricular segmentation methods in echocardiographic imaging.
}

\subsection{\modified{Contextualization-based approaches}}
\label{sec:contextualization_based_networks}

\modified{
In parallel, there has been an increasing interest in the computer vision community for deep learning methods based on contextualization
to improve classification~\cite{cvpr_wang_2017}, localization~\cite{nips_ren_fast_r_cnn_2015,cvpr_redmon_2016} and segmentation tasks~\cite{iccv_he_2017}. Specifically, these methods integrate surrounding information inside their pipeline to improve their overall performance.
}

\vspace*{0.1cm}
\modified{
\textit{\textbf{Region proposal methods}} apply the concept of contextualization in the image space. Specifically, these methods are based on the extraction of a region of interest (ROI) around the structures of concern before the segmentation step. One of the best performing approaches in computer vision is the Mask R-CNN method recently proposed by He \textit{et al.}. This approach provides the best current results in all three tracks of the COCO suite of challenges \cite{iccv_he_2017}. This network is mainly composed of three stages: \emph{i)} a region proposal network (RPN) which scans boxes distributed over the image area and finds the ones that contain objects; \emph{ii)} a classification network that scans each of the regions of interest proposed by the RPN and assigns them to different classes while refining the location and size of the bounding box to encapsulate the object; \emph{iii)} a convolutional network that takes the regions selected by the ROIs classifier and generates masks for them. In echocardiography, mainly two approaches have used this concept either for regression or segmentation. Ge \etal exploited contextualization before applying their regression network to estimate a set of clinical indices. In particular, a Res-circle network was applied to coherently detect the left ventricle centers over the cardiac cycle. Based on this information, a cropping strategy with pre-defined fixed dimensions was then applied to generate new images centered on the LV cavity. Leclerc \etal introduced a contextualization mechanism based on the multiplication of a binary map surrounding the union of the left ventricle and the myocardium (derived from a first network) with the input image in order to provide as input a pre-processed image without irrelevant information to a \unet~model that performs the segmentation of both the left ventricle and the myocardium simultaneously ~\cite{leclerc_ius_2019}. Results show that this method allows for a reduction of outliers in terms of segmentation results (from 20\% to 17\%) but unfortunately without any improvement in overall accuracy
}

%\vspace*{0.1cm}
\modified{
\textit{\textbf{Attention learning methods}} have also been successfully applied in medical imaging~\cite{oktay_midl_2018,media_vigneault_2018,media_pesce_2019,media_schlemper_2019}. Schlemper \etal developed a generic attention model to automatically learn to focus on target structures in medical imaging~\cite{media_schlemper_2019}. Based on attention gate modules that can be integrated in any existing CNN architecture~\cite{oktay_midl_2018}, the proposed formalism intrinsically promotes the suppression of irrelevant regions in an input image while highlighting salient features useful for a specific task. In parallel, Vigneault \etal proposed a dedicated CNN architecture for simultaneous localization and segmentation in cardiac MR imaging~\cite{media_vigneault_2018}. Their model is built around three stages: \emph{i)} an initial segmentation is performed on the input image; \emph{ii)} the features learned at the bottom layers are then used to predict the parameters of a spatial transformer network that transforms the input image into a canonical orientation~\cite{nips_jaderberg_2015}; \emph{iii)} a final segmentation is performed on the transformed image. To the best of our knowledge, no attention learning techniques have been applied so far for the segmentation of echocardiographic images.
}

\subsection{\modified{Objectives and contributions}}
\label{sec:objectives_and_contributions}

\modified{
%The study conducted in~\cite{Leclerc_tmi_2019} highlighted two interesting outputs: \emph{i)} the scores produced by a simple \unet~model are not much sensitive to the choice of hyper-parameters, which reinforces the quality of the results obtained by such architecture; \emph{ii)} the use of more sophisticated encoder-decoder architectures (\ie \mbox{U-Net++}~\cite{zhou2018}, stacked hourglasses network~\cite{newell2016} and anatomically constrained neural network~\cite{Oktay2018}) did not produce better results. Therefore, while \unet~ appears as a good choice for the segmentation of echocardiographic images, the improvement of its performance through the extension of its architecture is not straightforward.
}


==> sections/methodology_phd.tex <==
\section{Methodology}
\label{sec:methodology}

Based on the literature review carried out in the previous section, we decided to investigate in this paper the ability of attention learning based networks to improve the current best scores obtained from the CAMUS dataset. Indeed, CAMUS is the largest open access echocardiographic dataset, with an active evaluation website allowing a simple and objective comparison of state-of-the-art methods~\cite{Leclerc_tmi_2019}. 

\subsection{Overall strategy}
\label{sec:overall_strategy}

Based on the fact that the U-Net model already produces high-performance segmentation results in echocardiography, we decided to use this network to perform a first step of localization of the region of interest (\ie the left ventricle and the myocardium). The output of this step is then used either as a self-attention gating module for an attention network (referred to as RU-Net) or as a localization procedure for a multi-task network (referred to as LU-Net). The overall strategy of these two networks is provided in \Fig{}.

\subsection{RU-Net: an attention learning network}
\label{sec:ru_net}

%Inspired by the recent work of Schlemper \etal \cite{media_schlemper_2019}, we developed an attention gate method for the purpose of left ventricle and myocardium segmentation in 2D echocardiography. This method is based on a two-step strategy, as illustrated in \Fig{}.

\subsection{LU-Net: a multi-task network}
\label{sec:lu_net}

%Inspired by the recent work of Vigneault \etal \cite{media_vigneault_2018}, we also developed a multi-task network whose overall strategy is provided in \Fig{}. 


